Learning to Reason in 13 Parameters

Recent research has shown that language models can learn to \textit{reason}, often via reinforcement learning. Some work even trains low-rank parameterizations for reasoning, but conventional LoRA cannot scale below the model dimension. We question whether even rank=1 LoRA is necessary for learning to reason and propose TinyLoRA, a method for scaling low-rank adapters to sizes as small as one parameter. Within our new parameterization, we are able to train the 8B parameter size of Qwen2.5 to 91\% accuracy on GSM8K with only 13 trained parameters in bf16 (26 total bytes). We find this trend holds in general: we are able to recover 90\% of performance improvements while training $1000x$ fewer parameters across a suite of more difficult learning-to-reason benchmarks such as AIME, AMC, and MATH500. Notably, we are only able to achieve such strong performance with RL: models trained using SFT require $100-1000x$ larger updates to reach the same performance.

==> macros.tex <==
% \usepackage{algpseudocode}
% \usepackage[finalizecache,cachedir=.]{minted}
% \usepackage{algorithm}
% \usepackage{algorithmic}
% \usepackage{mathtools}
% \usepackage{wrapfig}
% \newcommand{\tva}{\mathbf{TV}_a}
% \newcommand{\eps}{\varepsilon}
% \newcommand{\adv}{\ensuremath{\mathbf{Adv}}}
% \newcommand{\tv}{\mathbf{TV}}
% % \newcommand{\cN}{\mathcal{N}}
% \newcommand{\nrm}[2]{\lVert #1 \rVert_{#2}}
% \newcommand{\pfix}[2]{{#1}_{\leq #2}}
\newcommand{\set}[1]{\{#1\}}
% \usepackage{microtype}
% \usepackage{graphicx}
% \usepackage{subfigure}
% \usepackage{booktabs} % for professional tables
% \usepackage{natbib}

% hyperref makes hyperlinks in the resulting PDF.
% If your build breaks (sometimes temporarily if a hyperlink spans a page)
% please comment out the following usepackage line and replace
% \usepackage{icml2021} with \usepackage[nohyperref]{icml2021} above.
% \usepackage{hyperref}

% Attempt to make hyperref and algorithmic work together better:
% \newcommand{\theHalgorithm}{\arabic{algorithm}}


% Use the following line for the initial blind version submitted for review:
% \usepackage{icml2022}

% \usepackage{amsmath}
% \usepackage{amssymb}
% \usepackage{amsthm}
% \usepackage{appendix}
% \usepackage{bbm}
% \usepackage{mathtools}
\newcounter{thm}

\newtheorem{theorem}[thm]{Theorem}
\newtheorem{lemma}[thm]{Lemma}
% \newtheorem{lemma}[thm]{Lemma}
% \newtheorem{corollary}[thm]{Corollary}
\newtheorem{proposition}[thm]{Proposition}
% \newtheorem{example}[thm]{Example}

% \newcommand{\fdp}{$f$-DP}
% \newcommand{\rvar}[1]{\mathbf{#1}}
\newtheorem{definition}[thm]{Definition}
% % \newtheorem{remark}[thm]{Remark}

% \newcommand\numberthis{\addtocounter{equation}{1}\tag{\theequation}}
% \newcommand{\prob}{\Pr}
% \newcommand{\andt}{\text{~and~} }
% \newcommand{\norm}{\mathcal{N}}
% \newcommand{\R}{\mathbb{R}}
% \DeclareMathOperator*{\E}{E}
% \newcommand{\Ex}{\E}
% \newcommand{\calD}{\mathcal{D}}
% \newcommand{\calM}{\mathcal{M}}
% \newcommand{\calA}{\mathcal{A}}
\newcommand{\acc}{\text{Acc}}
\newcommand{\Supp}{\mathsf{Supp}}
\newcommand{\SIM}{\mathrm{Sim}}
\newcommand{\SIMea}{\ensuremath{\mathrm{Sim}_{\exists\forall}}\xspace}
\newcommand{\datadist}{\cD}
\newcommand{\cg}{\mathcal{G}}

\NewDocumentCommand{\simdp}{O{$(\epsilon,\delta)$}}{%
  #1-SIM-DP\xspace%
}

\NewDocumentCommand{\simeadp}{O{$(\epsilon,\delta)$}}{%
  #1-SIM$_{\exists\forall}$-DP\xspace%
}
  
\NewDocumentCommand{\fDPi}{O{$(\epsilon,\delta)$}}{%
  #1-$\mathrm{DP}^\Psi_i$~%
}
\NewDocumentCommand{\fDPr}{O{$(\epsilon,\delta)$}}{%
  #1-$\mathrm{DP}^\Psi_r$~%
}
\NewDocumentCommand{\DPr}{O{$(\epsilon,\delta)$}}{%
  #1-$\mathrm{DP}_r$~%
}
\NewDocumentCommand{\DPi}{O{$(\epsilon,\delta)$}}{%
  #1-$\mathrm{DP}_i$~%
}
% \newcommand{\innerproduct}[2]{\langle #1, #2 \rangle}
% \newcommand{\hd}[2]{\textbf{HD}(#1, #2)}

% \newcommand{\audit}
% {\mathrm{audit}}

% \newcommand{\adv}{\text{Adv}}
% \newcommand{\N}{\mathbb{N}}
% \usepackage{etoolbox}
% \newcommand{\Ball}{\mathrm{Ball}}
% \newcommand{\bern}{\mathrm{Bernoulli}}
% Loop through each letter and define \cX command
\newcommand{\definecalletter}[1]{%
  \expandafter\newcommand\csname c#1\endcsname{\mathcal{#1}}%
}
\forcsvlist{\definecalletter}{A,B,C,D,E,F,G,H,I,J,K,L,M,N,O,P,Q,R,S,T,U,V,W,X,Y,Z}

\newcommand{\var}[1]{\mathbf{#1}}

% \DeclarePairedDelimiterX{\infdivx}[2]{(}{)}{%
%   #1\;\delimsize\|\;#2%
% }
\newcommand{\rdp}{D_\alpha\infdivx}
\newcommand{\kl}{\text{KL}\infdivx}
% \usepackage{xcolor}

\newcommand{\erf}{\mathrm{erf}}
\newcommand{\dummyfig}[1]{
  \centering
  \fbox{
    \begin{minipage}[c][0.33\textheight][c]{0.5\textwidth}
      \centering{#1}
    \end{minipage}
  }
}


% \usepackage{amsmath}
% \DeclareMathOperator*{\argmax}{arg\,max}
% \DeclareMathOperator*{\argmin}{arg\,min}

% \newif\ifcomments
% \commentstrue 
% % \commentsfalse

% \ifcomments
%     \newcommand{\saeed}[1]{{\color{red}Saeed: #1}}
%     \newcommand{\iden}[1]{{\color{purple}Iden: #1}}
%     \newcommand{\maxime}[1]{{\color{green}Maxime: #1}}
%     \newcommand{\ilya}[1]{{\color{blue}Ilya: #1}}
% \else 
%     \newcommand{\saeed}[1]{}
%     \newcommand{\iden}[1]{}
%     \newcommand{\maxime}[1]{}
%     \newcommand{\ilya}[1]{}
%     \renewcommand{\footnote}[1]{}
% \fi
